Tesla : an application for real-time data analysis in High Energy Physics

Upgrades to the LHCb computing infrastructure in the first long shutdown of the LHC have allowed for high quality decay information to be calculated by the software trigger making a separate offline event reconstruction unnecessary. Furthermore, the storage space of the triggered candidate is an order of magnitude smaller than the entire raw event that would otherwise need to be persisted. Tesla, following the LHCb renowned physicist naming convention, is an application designed to process the information calculated by the trigger, with the resulting output used to directly perform physics measurements.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

The \lhcb experiment, one of the four main detectors situated on the Large Hadron Collider in CERN, Geneva, specialises
in precision measurements of beauty and charm hadrons decays.
Large backgrounds are present at hadron colliders. 
At the nominal LHCb luminosity of $4\times10^{32}\, {\rm cm}^{-2}{\rm s}^{-1}$ during 2012 data taking at 8\tev, 
around 30\,k beauty ($b$) and 600\,k charm ($c$) hadron pairs pass through the detector each second. 
Each recorded collision is defined as an event that can possibly contain a decay of interest.
The most interesting $b$-hadron decays typically occur with decay probabilities of less than $10^{-5}$, whereas
a large fraction of $c$-hadron decays are retained for further study.
The efficient selection of beauty and charm decays from the $\mysim30$\,M proton-proton collisions per second is a significant Big Data challenge.

An innovative feature of the 
LHCb experiment is its approach to Big Data in the form of the High Level 
Trigger (HLT)~\cite{LHCb-DP-2012-004}. This is a software application designed to reduce the event
rate from 1\,M to $\mysim10$\,k events per second and is executed on an Event Filter 
Farm (EFF). The EFF is a computing cluster consisting of 1800 server nodes, with a combined storage space of 
5.2~PB. This can accommodate up to two weeks of LHCb data taking~\cite{LHCb-DP-2014-002} in nominal conditions. 
The HLT application reconstructs the particle trajectories of the event in real time, where real time is defined as the interval
between the collision in the detector and the moment the data are sent to permanent storage. The event reconstruction
in the EFF is denoted as the \emph{online reconstruction}.

In the LHCb data processing model of LHC Run-I (2010-2012), all events accepted by the 
HLT were sent to permanent offline storage containing all raw information from the detector.
An additional event reconstruction performed on the LHC Computing Grid~\cite{Stagni:2012nz}, denoted the \emph{offline reconstruction},
recreates particles in the event from the raw data using an improved detector calibration.

The upgrade of the computing infrastructure during the first long shutdown of the LHC (2013-2014), 
combined with efficient use of the EFF storage, provides resources for an online reconstruction in LHC Run-II (2015-2018) with a similar 
quality to that of the offline reconstruction.
This is achieved through real-time automated calculation of the final calibrations of the sub-detectors. 

With offline-quality information available at the HLT level,
it is possible to perform physics analyses with the information calculated by the HLT event reconstruction.
In the {\em Turbo stream}, a compact event record is written directly 
from the trigger and is prepared for physics analysis by the Tesla application.
This bypasses the offline reconstruction.
Reaching the ultimate precision of the \lhcb experiment already in real time as the data arrive
has the power to transform the experimental approach to 
processing large quantities of data. 

The data acquisition framework is described in Section~\ref{sec:trigger}.
An overview of the upgrades to the trigger and calibration
framework in Run-II is provided in Section~\ref{sec:run2}.
The implementation of the Turbo stream including that of the Tesla application is described in Section~\ref{sec:implementation},
followed by the future prospects of the data model in Section~\ref{sec:future}.

